Self-Attentive 3D Human Pose and Shape Estimation from Videos

We consider the task of estimating 3D human pose and shape from videos. While existing frame-based approaches have made significant progress, these methods are independently applied to each image, thereby often leading to inconsistent predictions. In this work, we present a video-based learning algorithm for 3D human pose and shape estimation. The key insights of our method are two-fold. First, to address the inconsistent temporal prediction issue, we exploit temporal information in videos and propose a self-attention module that jointly considers short-range and long-range dependencies across frames, resulting in temporally coherent estimations. Second, we model human motion with a forecasting module that allows the transition between adjacent frames to be smooth. We evaluate our method on the 3DPW, MPI-INF-3DHP, and Human3.6M datasets. Extensive experimental results show that our algorithm performs favorably against the state-of-the-art methods.

==> setup/graphicspath.tex <==
\graphicspath{{figure}, {example}}


==> setup/macros.tex <==
% Macros - Jia-Bin Huang (jbhuang@vt.edu)

\renewcommand{\baselinestretch}{1}       % for squeezing the draft into the page limit, do not use

% =========================================
% Useful macros
% =========================================

% Latin abbreviations
\newcommand{\bbR}{{\mathbb{R}}}

\newcommand{\first}[1]{{\color{blue}\textbf{#1}}}
\newcommand{\second}[1]{{\color{red}\underline{#1}}}

% Math related
\DeclareMathOperator*{\argmin}{\arg\!\min} 
\DeclareMathOperator*{\argmax}{\arg\!\max}

% Consistent margin adjustment for paragraphs, figures, and sections
\newlength\paramargin
\newlength\figmargin
\newlength\secmargin
\newlength\figcapmargin
\newlength\twoimg
\newlength\threeimg
\newlength\fourimg
\newlength\fiveimg
\newlength\siximg
\newlength\sevenimg
\newlength\eightimg

\setlength{\secmargin}{0.0mm}
\setlength{\paramargin}{-3.0mm}
\setlength{\figmargin}{0.0mm}
\setlength{\figcapmargin}{0.0mm}

\newcommand{\heading}[1]
{\noindent\textbf{#1}}

\newcommand{\red}{\textcolor{red}}
\newcommand{\blue}{\textcolor{blue}}

% minipage
\newcommand{\mpage}[2]
{
\begin{minipage}{#1\textwidth}\centering
#2
\end{minipage}
}

% mini-figure
\newcommand{\mfigure}[2]
{
\begin{subfigure}[t]{#1\linewidth} \centering
\includegraphics[width=\linewidth]{#2}
\end{subfigure}
}

\newcommand{\etal}{\textit{et~al}\mbox{.}}

% Comments
\long\def\ignorethis#1{}
\newcommand {\ycchen}[1]{{\color{blue}\textbf{Yun-Chun: }#1}\normalfont}
\newcommand {\mhyang}[1]{{\color{red}\textbf{Ming-Hsuan: }#1}\normalfont}
\newcommand {\todo}{{\textbf{\color{red}[TO-DO]\_}}}
\def\newtext#1{\textcolor{blue}{#1}}
\def\modtext#1{\textcolor{red}{#1}}
\newcommand{\note}[1]{{\it\color{blue} #1}}

\newcommand{\tb}[1]{\textbf{#1}}
\newcommand{\mb}[1]{\mathbf{#1}}

\newcommand{\jbox}[2]{
  \fbox{%
  	\begin{minipage}{#1}%
  		\hfill\vspace{#2}%
  	\end{minipage}%
  }}

\newcommand{\jblock}[2]{%
	\begin{minipage}[t]{#1}\vspace{0cm}\centering%
	#2%
	\end{minipage}%
}



==> setup/package.tex <==
% Figures
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{float}
\usepackage{caption}	% makes captions ragged right - thanks to Bryce Lobdell
\usepackage{lscape}                                      

% Algorithm
\usepackage[lined,ruled,linesnumbered]{algorithm2e}

% Table and list
\usepackage{booktabs}                   % Publication quality tables
\usepackage{multirow}

\usepackage{paralist}
\usepackage{enumitem}

% \usepackage[numbers, sort]{natbib}
\usepackage{natbib}
% \usepackage{cite}


% Math
\usepackage{bm}                          % Make bold, italic math symbols
\usepackage{epsfig}                      % for figures
\usepackage{graphicx}                  % another package that works for figures
\usepackage{times}
%\usepackage{mathptmx}
\usepackage{mathtools}
\usepackage{amssymb,amsmath}   % Short math guide for LaTeX ftp://ftp.ams.org/pub/tex/doc/amsmath/short-math-guide.pdf

% Fonts
\usepackage{units}
\usepackage{color}

% \usepackage{movie15}

% Comments
\usepackage{comment}

% Hyperlinks
\usepackage{url}  % Hyphenation of URLs.
% \usepackage[pagebackref=true,breaklinks=true,colorlinks,urlcolor=blue,citecolor=blue,linkcolor=blue,bookmarks=false]{hyperref}
\usepackage[breaklinks=true,colorlinks,urlcolor=blue,citecolor=blue,linkcolor=blue,bookmarks=false]{hyperref}

% \usepackage{slashbox}
\usepackage{xspace}
% \usepackage[table]{xcolor}
% \usepackage{setspace}


\usepackage{nicefrac}
\usepackage{microtype}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts

% \usepackage{times,color}
% \usepackage{parskip}
% %\usepackage{epsfig}
% %\usepackage{psfig}
% %\usepackage[pdftex]{graphicx} % new acmsiggraph.cls
% \usepackage{ifthen}
% %\usepackage[draft]{hyperref} % new acmsiggraph.cls
% \usepackage{float}
% \usepackage{alltt}
% \usepackage{mathenv}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{amsthm}
% %\usepackage{rotating}
% \usepackage{newlfont} % for Box
% %\usepackage{ulem}
% \usepackage{floatflt}
% \usepackage{wrapfig}
% \usepackage{fixltx2e}
% \usepackage{subfig} % for subfloat
% \usepackage{multirow}
% \usepackage{cleveref}
% \usepackage{algorithmic}
% \usepackage{CJKutf8} % Chinese

